Descriminative-Generative Custom Tokens for Vision-Language Models

This paper explores the possibility of learning custom tokens for representing new concepts in Vision-Language Models (VLMs). Our aim is to learn tokens that can be effective for both discriminative and generative tasks while composing well with words to form new input queries. The targeted concept is specified in terms of a small set of images and a parent concept described using text. We operate on CLIP text features and propose to use a combination of a textual inversion loss and a classification loss to ensure that text features of the learned token are aligned with image features of the concept in the CLIP embedding space. We restrict the learned token to a low-dimensional subspace spanned by tokens for attributes that are appropriate for the given super-class. These modifications improve the quality of compositions of the learned token with natural language for generating new scenes. Further, we show that learned custom tokens can be used to form queries for text-to-image retrieval task, and also have the important benefit that composite queries can be visualized to ensure that the desired concept is faithfully encoded. Based on this, we introduce the method of Generation Aided Image Retrieval, where the query is modified at inference time to better suit the search intent. On the DeepFashion2 dataset, our method improves Mean Reciprocal Retrieval (MRR) over relevant baselines by 7%.

==> eccv <==
@String(PAMI = {IEEE Trans. Pattern Anal. Mach. Intell.})
@String(IJCV = {Int. J. Comput. Vis.})
@String(CVPR= {IEEE Conf. Comput. Vis. Pattern Recog.})
@String(ICCV= {Int. Conf. Comput. Vis.})
@String(ECCV= {Eur. Conf. Comput. Vis.})
@String(NIPS= {Adv. Neural Inform. Process. Syst.})
@String(ICPR = {Int. Conf. Pattern Recog.})
@String(BMVC= {Brit. Mach. Vis. Conf.})
@String(TOG= {ACM Trans. Graph.})
@String(TIP  = {IEEE Trans. Image Process.})
@String(TVCG  = {IEEE Trans. Vis. Comput. Graph.})
@String(TMM  = {IEEE Trans. Multimedia})
@String(ACMMM= {ACM Int. Conf. Multimedia})
@String(ICME = {Int. Conf. Multimedia and Expo})
@String(ICASSP=	{ICASSP})
@String(ICIP = {IEEE Int. Conf. Image Process.})
@String(ACCV  = {ACCV})
@String(ICLR = {Int. Conf. Learn. Represent.})
@String(IJCAI = {IJCAI})
@String(PR   = {Pattern Recognition})
@String(AAAI = {AAAI})
@String(CVPRW= {IEEE Conf. Comput. Vis. Pattern Recog. Worksh.})
@String(CSVT = {IEEE Trans. Circuit Syst. Video Technol.})

@String(SPL	= {IEEE Sign. Process. Letters})
@String(VR   = {Vis. Res.})
@String(JOV	 = {J. Vis.})
@String(TVC  = {The Vis. Comput.})
@String(JCST  = {J. Comput. Sci. Tech.})
@String(CGF  = {Comput. Graph. Forum})
@String(CVM = {Computational Visual Media})


@String(PAMI  = {IEEE TPAMI})
@String(IJCV  = {IJCV})
@String(CVPR  = {CVPR})
@String(ICCV  = {ICCV})
@String(ECCV  = {ECCV})
@String(NIPS  = {NeurIPS})
@String(ICPR  = {ICPR})
@String(BMVC  =	{BMVC})
@String(TOG   = {ACM TOG})
@String(TIP   = {IEEE TIP})
@String(TVCG  = {IEEE TVCG})
@String(TCSVT = {IEEE TCSVT})
@String(TMM   =	{IEEE TMM})
@String(ACMMM = {ACM MM})
@String(ICME  =	{ICME})
@String(ICASSP=	{ICASSP})
@String(ICIP  = {ICIP})
@String(ACCV  = {ACCV})
@String(ICLR  = {ICLR})
@String(IJCAI = {IJCAI})
@String(PR = {PR})
@String(AAAI = {AAAI})
@String(CVPRW= {CVPRW})
@String(CSVT = {IEEE TCSVT})


@inproceedings{ddpm,
 author = {Ho, Jonathan and Jain, Ajay and Abbeel, Pieter},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {H. Larochelle and M. Ranzato and R. Hadsell and M.F. Balcan and H. Lin},
 pages = {6840--6851},
 publisher = {Curran Associates, Inc.},
 title = {Denoising Diffusion Probabilistic Models},
 url = {https://proceedings.neurips.cc/paper_files/paper/2020/file/4c5bcfec8584af0d967f1ab10179ca4b-Paper.pdf},
 volume = {33},
 year = {2020}
}

@Inproceedings{Trager2023,
 author = {Matthew Trager and Pramuditha Perera and Luca Zancato and Alessandro Achille and Parminder Bhatia and Stefano Soatto},
 title = {Linear spaces of meanings: Compositional structures in vision-language models},
 year = {2023},
 url = {https://www.amazon.science/publications/linear-spaces-of-meanings-compositional-structures-in-vision-language-models},
 booktitle = {ICCV 2023},
}

@article{zhou2022coop,
    title={Learning to Prompt for Vision-Language Models},
    author={Zhou, Kaiyang and Yang, Jingkang and Loy, Chen Change and Liu, Ziwei},
    journal={International Journal of Computer Vision (IJCV)},
    year={2022}
}

@inproceedings{
textinversion,
title={An Image is Worth One Word: Personalizing Text-to-Image Generation using Textual Inversion},
author={Rinon Gal and Yuval Alaluf and Yuval Atzmon and Or Patashnik and Amit Haim Bermano and Gal Chechik and Daniel Cohen-or},
booktitle={The Eleventh International Conference on Learning Representations },
year={2023},
url={https://openreview.net/forum?id=NAQvF08TcyG}
}

@inproceedings{devlin-etal-2019-bert,
    title = "{BERT}: Pre-training of Deep Bidirectional Transformers for Language Understanding",
    author = "Devlin, Jacob  and
      Chang, Ming-Wei  and
      Lee, Kenton  and
      Toutanova, Kristina",
    booktitle = "Proceedings of the 2019 Conference of the North {A}merican Chapter of the Association for Computational Linguistics: Human Language Technologies, Volume 1 (Long and Short Papers)",
    month = jun,
    year = "2019",
    address = "Minneapolis, Minnesota",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/N19-1423",
    doi = "10.18653/v1/N19-1423",
    pages = "4171--4186",
    abstract = "We introduce a new language representation model called BERT, which stands for Bidirectional Encoder Representations from Transformers. Unlike recent language representation models (Peters et al., 2018a; Radford et al., 2018), BERT is designed to pre-train deep bidirectional representations from unlabeled text by jointly conditioning on both left and right context in all layers. As a result, the pre-trained BERT model can be fine-tuned with just one additional output layer to create state-of-the-art models for a wide range of tasks, such as question answering and language inference, without substantial task-specific architecture modifications. BERT is conceptually simple and empirically powerful. It obtains new state-of-the-art results on eleven natural language processing tasks, including pushing the GLUE score to 80.5 (7.7 point absolute improvement), MultiNLI accuracy to 86.7{\%} (4.6{\%} absolute improvement), SQuAD v1.1 question answering Test F1 to 93.2 (1.5 point absolute improvement) and SQuAD v2.0 Test F1 to 83.1 (5.1 point absolute improvement).",
}



@misc{model_zoo,
  doi = {10.48550/ARXIV.2102.00084},
  url = {https://arxiv.org/abs/2102.00084},
  author = {Deshpande, Aditya and Achille, Alessandro and Ravichandran, Avinash and Li, Hao and Zancato, Luca and Fowlkes, Charless and Bhotika, Rahul and Soatto, Stefano and Perona, Pietro},
  keywords = {Computer Vision and Pattern Recognition (cs.CV), Machine Learning (cs.LG), FOS: Computer and information sciences, FOS: Computer and information sciences},
  title = {A linearized framework and a new benchmark for model selection for fine-tuning},
  publisher = {arXiv},
  year = {2021},
  copyright = {arXiv.org perpetual, non-exclusive license}
}


@misc{adaContrast,
  doi = {10.48550/ARXIV.2204.10377},
  url = {https://arxiv.org/abs/2204.10377},
  author = {Chen, Dian and Wang, Dequan and Darrell, Trevor and Ebrahimi, Sayna},
  keywords = {Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  title = {Contrastive Test-Time Adaptation},
  publisher = {arXiv},
  year = {2022},
  copyright = {Creative Commons Attribution 4.0 International}
}

@misc{retrieval_augmented_classification,
  doi = {10.48550/ARXIV.2202.11233},
  url = {https://arxiv.org/abs/2202.11233},
  author = {Long, Alexander and Yin, Wei and Ajanthan, Thalaiyasingam and Nguyen, Vu and Purkait, Pulak and Garg, Ravi and Blair, Alan and Shen, Chunhua and Hengel, Anton van den},
  keywords = {Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  title = {Retrieval Augmented Classification for Long-Tail Visual Recognition},
  publisher = {arXiv},
  year = {2022},
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@misc{LQF,
  doi = {10.48550/ARXIV.2012.11140},
  url = {https://arxiv.org/abs/2012.11140},
  author = {Achille, Alessandro and Golatkar, Aditya and Ravichandran, Avinash and Polito, Marzia and Soatto, Stefano},
  keywords = {Machine Learning (cs.LG), Computer Vision and Pattern Recognition (cs.CV), Machine Learning (stat.ML), FOS: Computer and information sciences, FOS: Computer and information sciences},
  title = {LQF: Linear Quadratic Fine-Tuning},
  publisher = {arXiv},
  year = {2020},
  copyright = {arXiv.org perpetual, non-exclusive license}
}


@misc{RETRO,
  doi = {10.48550/ARXIV.2112.04426},
  url = {https://arxiv.org/abs/2112.04426},
  author = {Borgeaud, Sebastian and Mensch, Arthur and Hoffmann, Jordan and Cai, Trevor and Rutherford, Eliza and Millican, Katie and Driessche, George van den and Lespiau, Jean-Baptiste and Damoc, Bogdan and Clark, Aidan and Casas, Diego de Las and Guy, Aurelia and Menick, Jacob and Ring, Roman and Hennigan, Tom and Huang, Saffron and Maggiore, Loren and Jones, Chris and Cassirer, Albin and Brock, Andy and Paganini, Michela and Irving, Geoffrey and Vinyals, Oriol and Osindero, Simon and Simonyan, Karen and Rae, Jack W. and Elsen, Erich and Sifre, Laurent},
  keywords = {Computation and Language (cs.CL), Machine Learning (cs.LG), FOS: Computer and information sciences, FOS: Computer and information sciences},
  title = {Improving language models by retrieving from trillions of tokens},
  publisher = {arXiv},
  year = {2021},
  copyright = {Creative Commons Attribution 4.0 International}
}





@misc{ViT,
  doi = {10.48550/ARXIV.2010.11929},
  
  url = {https://arxiv.org/abs/2010.11929},
  
  author = {Dosovitskiy, Alexey and Beyer, Lucas and Kolesnikov, Alexander and Weissenborn, Dirk and Zhai, Xiaohua and Unterthiner, Thomas and Dehghani, Mostafa and Minderer, Matthias and Heigold, Georg and Gelly, Sylvain and Uszkoreit, Jakob and Houlsby, Neil},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), Artificial Intelligence (cs.AI), Machine Learning (cs.LG), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {An Image is Worth 16x16 Words: Transformers for Image Recognition at Scale},
  
  publisher = {arXiv},
  
  year = {2020},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@misc{ConvNext,
  doi = {10.48550/ARXIV.2201.03545},
  
  url = {https://arxiv.org/abs/2201.03545},
  
  author = {Liu, Zhuang and Mao, Hanzi and Wu, Chao-Yuan and Feichtenhofer, Christoph and Darrell, Trevor and Xie, Saining},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {A ConvNet for the 2020s},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {Creative Commons Attribution 4.0 International}
}


@misc{prompt_continual_learning,
  doi = {10.48550/ARXIV.2112.08654},
  
  url = {https://arxiv.org/abs/2112.08654},
  
  author = {Wang, Zifeng and Zhang, Zizhao and Lee, Chen-Yu and Zhang, Han and Sun, Ruoxi and Ren, Xiaoqi and Su, Guolong and Perot, Vincent and Dy, Jennifer and Pfister, Tomas},
  
  keywords = {Machine Learning (cs.LG), Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Learning to Prompt for Continual Learning},
  
  publisher = {arXiv},
  
  year = {2021},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@article{continual_learning_survey,
	doi = {10.1109/tpami.2021.3057446},
  
	url = {https://doi.org/10.1109%2Ftpami.2021.3057446},
  
	year = 2021,
	publisher = {Institute of Electrical and Electronics Engineers ({IEEE})},
  
	pages = {1--1},
  
	author = {Matthias Delange and Rahaf Aljundi and Marc Masana and Sarah Parisot and Xu Jia and Ales Leonardis and Greg Slabaugh and Tinne Tuytelaars},
  
	title = {A continual learning survey: Defying forgetting in classification tasks},
  
	journal = {{IEEE} Transactions on Pattern Analysis and Machine Intelligence}
}

@misc{online_continual_learning,
  doi = {10.48550/ARXIV.2101.10423},
  
  url = {https://arxiv.org/abs/2101.10423},
  
  author = {Mai, Zheda and Li, Ruiwen and Jeong, Jihwan and Quispe, David and Kim, Hyunwoo and Sanner, Scott},
  
  keywords = {Machine Learning (cs.LG), Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Online Continual Learning in Image Classification: An Empirical Survey},
  
  publisher = {arXiv},
  
  year = {2021},
  
  copyright = {Creative Commons Attribution 4.0 International}
}

@misc{mixed_privacy_forgetting_aditya,
  doi = {10.48550/ARXIV.2012.13431},
  
  url = {https://arxiv.org/abs/2012.13431},
  
  author = {Golatkar, Aditya and Achille, Alessandro and Ravichandran, Avinash and Polito, Marzia and Soatto, Stefano},
  
  keywords = {Machine Learning (cs.LG), Artificial Intelligence (cs.AI), Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Mixed-Privacy Forgetting in Deep Networks},
  
  publisher = {arXiv},
  
  year = {2020},
  
  copyright = {Creative Commons Attribution 4.0 International}
}

@misc{forgetting_data_deletion,
  doi = {10.48550/ARXIV.1907.05012},
  
  url = {https://arxiv.org/abs/1907.05012},
  
  author = {Ginart, Antonio and Guan, Melody Y. and Valiant, Gregory and Zou, James},
  
  keywords = {Machine Learning (cs.LG), Machine Learning (stat.ML), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Making AI Forget You: Data Deletion in Machine Learning},
  
  publisher = {arXiv},
  
  year = {2019},
  
  copyright = {Creative Commons Attribution Share Alike 4.0 International}
}

@misc{test_time_training,
  doi = {10.48550/ARXIV.1909.13231},
  
  url = {https://arxiv.org/abs/1909.13231},
  
  author = {Sun, Yu and Wang, Xiaolong and Liu, Zhuang and Miller, John and Efros, Alexei A. and Hardt, Moritz},
  
  keywords = {Machine Learning (cs.LG), Computer Vision and Pattern Recognition (cs.CV), Machine Learning (stat.ML), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Test-Time Training with Self-Supervision for Generalization under Distribution Shifts},
  
  publisher = {arXiv},
  
  year = {2019},
  
  copyright = {Creative Commons Zero v1.0 Universal}
}


@misc{tent,
  doi = {10.48550/ARXIV.2006.10726},
  
  url = {https://arxiv.org/abs/2006.10726},
  
  author = {Wang, Dequan and Shelhamer, Evan and Liu, Shaoteng and Olshausen, Bruno and Darrell, Trevor},
  
  keywords = {Machine Learning (cs.LG), Computer Vision and Pattern Recognition (cs.CV), Machine Learning (stat.ML), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Tent: Fully Test-time Adaptation by Entropy Minimization},
  
  publisher = {arXiv},
  
  year = {2020},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@misc{Neural_Turing_Machine,
  doi = {10.48550/ARXIV.1410.5401},
  
  url = {https://arxiv.org/abs/1410.5401},
  
  author = {Graves, Alex and Wayne, Greg and Danihelka, Ivo},
  
  keywords = {Neural and Evolutionary Computing (cs.NE), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Neural Turing Machines},
  
  publisher = {arXiv},
  
  year = {2014},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@misc{anomaly_detection_retrieval,
  doi = {10.48550/ARXIV.1904.02639},
  
  url = {https://arxiv.org/abs/1904.02639},
  
  author = {Gong, Dong and Liu, Lingqiao and Le, Vuong and Saha, Budhaditya and Mansour, Moussa Reda and Venkatesh, Svetha and Hengel, Anton van den},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Memorizing Normality to Detect Anomaly: Memory-augmented Deep Autoencoder for Unsupervised Anomaly Detection},
  
  publisher = {arXiv},
  
  year = {2019},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@misc{retrieval_diffusion_models,
  doi = {10.48550/ARXIV.2209.14491},
  
  url = {https://arxiv.org/abs/2209.14491},
  
  author = {Chen, Wenhu and Hu, Hexiang and Saharia, Chitwan and Cohen, William W.},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), Artificial Intelligence (cs.AI), Machine Learning (cs.LG), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Re-Imagen: Retrieval-Augmented Text-to-Image Generator},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@misc{MEMO_test_time_adaptation,
  doi = {10.48550/ARXIV.2110.09506},
  
  url = {https://arxiv.org/abs/2110.09506},
  
  author = {Zhang, Marvin and Levine, Sergey and Finn, Chelsea},
  
  keywords = {Machine Learning (cs.LG), Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {MEMO: Test Time Robustness via Adaptation and Augmentation},
  
  publisher = {arXiv},
  
  year = {2021},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}


@INPROCEEDINGS{mit67recognizing,  author={Quattoni, Ariadna and Torralba, Antonio},  booktitle={2009 IEEE Conference on Computer Vision and Pattern Recognition},   title={Recognizing indoor scenes},   year={2009},  volume={},  number={},  pages={413-420},  doi={10.1109/CVPR.2009.5206537}}

@techreport{WahCUB_200_2011,
	Title = {},
	Author = {Wah, C. and Branson, S. and Welinder, P. and Perona, P. and Belongie, S.},
	Year = {2011},
	Institution = {California Institute of Technology},
	Number = {CNS-TR-2011-001}
}

@techreport{maji13fine-grained,
   title         = {Fine-Grained Visual Classification of Aircraft},
   author        = {S. Maji and J. Kannala and E. Rahtu
                    and M. Blaschko and A. Vedaldi},
   year          = {2013},
   archivePrefix = {arXiv},
   eprint        = {1306.5151},
   primaryClass  = "cs-cv",
}

@InProceedings{Nilsback06,
  author       = "Maria-Elena Nilsback and Andrew Zisserman",
  title        = "A Visual Vocabulary for Flower Classification",
  booktitle    = "IEEE Conference on Computer Vision and Pattern Recognition",
  volume       = "2",
  pages        = "1447--1454",
  year         = "2006",
}

 @misc{griffin_holub_perona_2022, title={Caltech 256}, DOI={10.22002/D1.20087}, abstractNote={We introduce a challenging set of 256 object categories containing a total of 30607 images. The original Caltech-101 was collected by choosing a set of object categories, downloading examples from Google Images and then manually screening out all images that did not fit the category. Caltech-256 is collected in a similar manner with several improvements: a) the number of categories is more than doubled, b) the minimum number of images in any category is increased from 31 to 80, c) artifacts due to image rotation are avoided and d) a new and larger clutter category is introduced for testing background rejection. We suggest several testing paradigms to measure classification performance, then benchmark the dataset using two simple metrics as well as a state-of-the-art spatial pyramid matching algorithm. Finally we use the clutter category to train an interest detector which rejects uninformative background regions.}, publisher={CaltechDATA}, author={Griffin and Holub and Perona}, year={2022}, month={Apr} }
 
 @InProceedings{parkhi12a,
  author       = "Omkar M. Parkhi and Andrea Vedaldi and Andrew Zisserman and C. V. Jawahar",
  title        = "Cats and Dogs",
  booktitle    = "IEEE Conference on Computer Vision and Pattern Recognition",
  year         = "2012",
}

@misc{VISDA,
  doi = {10.48550/ARXIV.1710.06924},
  
  url = {https://arxiv.org/abs/1710.06924},
  
  author = {Peng, Xingchao and Usman, Ben and Kaushik, Neela and Hoffman, Judy and Wang, Dequan and Saenko, Kate},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {VisDA: The Visual Domain Adaptation Challenge},
  
  publisher = {arXiv},
  
  year = {2017},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}


@misc{domainnet,
  doi = {10.48550/ARXIV.1812.01754},
  
  url = {https://arxiv.org/abs/1812.01754},
  
  author = {Peng, Xingchao and Bai, Qinxun and Xia, Xide and Huang, Zijun and Saenko, Kate and Wang, Bo},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Moment Matching for Multi-Source Domain Adaptation},
  
  publisher = {arXiv},
  
  year = {2018},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}


@inproceedings{stanfordcars,
  title = {3D Object Representations for Fine-Grained Categorization},
  booktitle = {4th International IEEE Workshop on  3D Representation and Recognition (3dRR-13)},
  year = {2013},
  address = {Sydney, Australia},
  author = {Jonathan Krause and Michael Stark and Jia Deng and Li Fei-Fei}
}

@article{bell15minc,
	author = "Sean Bell and Paul Upchurch and Noah Snavely and Kavita Bala",
	title = "Material Recognition in the Wild with the Materials in Context Database",
	journal = "Computer Vision and Pattern Recognition (CVPR)",
	year = "2015",
}

@inproceedings{stanforddogs,
author = "Aditya Khosla and Nityananda Jayadevaprakash and Bangpeng Yao and Li Fei-Fei",
title = "Novel Dataset for Fine-Grained Image Categorization",
booktitle = "First Workshop on Fine-Grained Visual Categorization, IEEE Conference on Computer Vision and Pattern Recognition",
year = "2011",
month = "June",
address = "Colorado Springs, CO",
}

@inproceedings{imagenet_cvpr09,
        AUTHOR = {Deng, J. and Dong, W. and Socher, R. and Li, L.-J. and Li, K. and Fei-Fei, L.},
        TITLE = {{ImageNet: A Large-Scale Hierarchical Image Database}},
        BOOKTITLE = {CVPR09},
        YEAR = {2009},
        BIBSOURCE = "http://www.image-net.org/papers/imagenet_cvpr09.bib"}


@article{iNaturalist_HornASSAPB17,
  author    = {Grant Van Horn and
               Oisin {Mac Aodha} and
               Yang Song and
               Alexander Shepard and
               Hartwig Adam and
               Pietro Perona and
               Serge J. Belongie},
  title     = {The iNaturalist Challenge 2017 Dataset},
  journal   = {CoRR},
  volume    = {abs/1707.06642},
  year      = {2017},
  url       = {http://arxiv.org/abs/1707.06642},
  archivePrefix = {arXiv},
  eprint    = {1707.06642},
  timestamp = {Mon, 13 Aug 2018 16:48:58 +0200},
}

@inproceedings{food101,
  title = {Food-101 -- Mining Discriminative Components with Random Forests},
  author = {Bossard, Lukas and Guillaumin, Matthieu and Van Gool, Luc},
  booktitle = {European Conference on Computer Vision},
  year = {2014}
}

@inproceedings{logo2k,
	title = {Logo-2K+: A Large-Scale Logo Dataset for Scalable Logo Classification},
	journal = {AAAI Conference on Artificial Intelligence (AAAI)},
	year = {2019},
	note = {\&nbsp;\&nbsp;\&nbsp;},
	abstract = {\&nbsp;\&nbsp;\&nbsp;},
	author = {Wang, J. and W. Min and S. Hou and Ma, S. and Y. Zheng and Wang, H. and S. Jiang}
}

@ARTICLE{nwpu_resisc45, author={G. {Cheng} and J. {Han} and X. {Lu}}, journal={Proceedings of the IEEE}, title={Remote Sensing Image Scene Classification: Benchmark and State of the Art}, year={2017}, volume={105}, number={10}, pages={1865-1883},}

@misc{imaterialist,
author={MalongTech},
title = {Imaterialist Dataset, https://github.com/MalongTech/imaterialist-product-2019},
url = {https://github.com/MalongTech/imaterialist-product-2019}
}

@misc{SHOT,
  doi = {10.48550/ARXIV.2002.08546},
  
  url = {https://arxiv.org/abs/2002.08546},
  
  author = {Liang, Jian and Hu, Dapeng and Feng, Jiashi},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), Machine Learning (cs.LG), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Do We Really Need to Access the Source Data? Source Hypothesis Transfer for Unsupervised Domain Adaptation},
  
  publisher = {arXiv},
  
  year = {2020},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}


@misc{dino,
  doi = {10.48550/ARXIV.2104.14294},
  
  url = {https://arxiv.org/abs/2104.14294},
  
  author = {Caron, Mathilde and Touvron, Hugo and Misra, Ishan and Jégou, Hervé and Mairal, Julien and Bojanowski, Piotr and Joulin, Armand},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Emerging Properties in Self-Supervised Vision Transformers},
  
  publisher = {arXiv},
  
  year = {2021},
  
  copyright = {Creative Commons Attribution 4.0 International}
}


@misc{divide_and_contrast,
  doi = {10.48550/ARXIV.2105.08054},
  
  url = {https://arxiv.org/abs/2105.08054},
  
  author = {Tian, Yonglong and Henaff, Olivier J. and Oord, Aaron van den},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Divide and Contrast: Self-supervised Learning from Uncurated Data},
  
  publisher = {arXiv},
  
  year = {2021},
  
  copyright = {Creative Commons Attribution 4.0 International}
}


@misc{thinking_fast_and_slow,
  doi = {10.48550/ARXIV.2103.16553},
  
  url = {https://arxiv.org/abs/2103.16553},
  
  author = {Miech, Antoine and Alayrac, Jean-Baptiste and Laptev, Ivan and Sivic, Josef and Zisserman, Andrew},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Thinking Fast and Slow: Efficient Text-to-Visual Retrieval with Transformers},
  
  publisher = {arXiv},
  
  year = {2021},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@misc{retrieval_generative_models,
  doi = {10.48550/ARXIV.2204.11824},
  
  url = {https://arxiv.org/abs/2204.11824},
  
  author = {Blattmann, Andreas and Rombach, Robin and Oktay, Kaan and Müller, Jonas and Ommer, Björn},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Semi-Parametric Neural Image Synthesis},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@misc{MoCo,
  doi = {10.48550/ARXIV.1911.05722},
  
  url = {https://arxiv.org/abs/1911.05722},
  
  author = {He, Kaiming and Fan, Haoqi and Wu, Yuxin and Xie, Saining and Girshick, Ross},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Momentum Contrast for Unsupervised Visual Representation Learning},
  
  publisher = {arXiv},
  
  year = {2019},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@misc{simclr,
  doi = {10.48550/ARXIV.2002.05709},
  
  url = {https://arxiv.org/abs/2002.05709},
  
  author = {Chen, Ting and Kornblith, Simon and Norouzi, Mohammad and Hinton, Geoffrey},
  
  keywords = {Machine Learning (cs.LG), Computer Vision and Pattern Recognition (cs.CV), Machine Learning (stat.ML), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {A Simple Framework for Contrastive Learning of Visual Representations},
  
  publisher = {arXiv},
  
  year = {2020},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@misc{supcon,
  doi = {10.48550/ARXIV.2004.11362},
  
  url = {https://arxiv.org/abs/2004.11362},
  
  author = {Khosla, Prannay and Teterwak, Piotr and Wang, Chen and Sarna, Aaron and Tian, Yonglong and Isola, Phillip and Maschinot, Aaron and Liu, Ce and Krishnan, Dilip},
  
  keywords = {Machine Learning (cs.LG), Computer Vision and Pattern Recognition (cs.CV), Machine Learning (stat.ML), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Supervised Contrastive Learning},
  
  publisher = {arXiv},
  
  year = {2020},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@misc{comatch,
  doi = {10.48550/ARXIV.2011.11183},
  
  url = {https://arxiv.org/abs/2011.11183},
  
  author = {Li, Junnan and Xiong, Caiming and Hoi, Steven},
  
  keywords = {Machine Learning (cs.LG), Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {CoMatch: Semi-supervised Learning with Contrastive Graph Regularization},
  
  publisher = {arXiv},
  
  year = {2020},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}


@misc{meta_opt_net,
  doi = {10.48550/ARXIV.1904.03758},
  
  url = {https://arxiv.org/abs/1904.03758},
  
  author = {Lee, Kwonjoon and Maji, Subhransu and Ravichandran, Avinash and Soatto, Stefano},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), Machine Learning (cs.LG), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Meta-Learning with Differentiable Convex Optimization},
  
  publisher = {arXiv},
  
  year = {2019},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}


@misc{R2D2,
  doi = {10.48550/ARXIV.1805.08136},
  
  url = {https://arxiv.org/abs/1805.08136},
  
  author = {Bertinetto, Luca and Henriques, João F. and Torr, Philip H. S. and Vedaldi, Andrea},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), Machine Learning (cs.LG), Machine Learning (stat.ML), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Meta-learning with differentiable closed-form solvers},
  
  publisher = {arXiv},
  
  year = {2018},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@misc{CAN,
  doi = {10.48550/ARXIV.1901.00976},
  
  url = {https://arxiv.org/abs/1901.00976},
  
  author = {Kang, Guoliang and Jiang, Lu and Yang, Yi and Hauptmann, Alexander G},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Contrastive Adaptation Network for Unsupervised Domain Adaptation},
  
  publisher = {arXiv},
  
  year = {2019},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@misc{MCC,
  doi = {10.48550/ARXIV.1912.03699},
  
  url = {https://arxiv.org/abs/1912.03699},
  
  author = {Jin, Ying and Wang, Ximei and Long, Mingsheng and Wang, Jianmin},
  
  keywords = {Machine Learning (cs.LG), Computer Vision and Pattern Recognition (cs.CV), Machine Learning (stat.ML), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Minimum Class Confusion for Versatile Domain Adaptation},
  
  publisher = {arXiv},
  
  year = {2019},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@misc{OFA,
  doi = {10.48550/ARXIV.2202.03052},
  
  url = {https://arxiv.org/abs/2202.03052},
  
  author = {Wang, Peng and Yang, An and Men, Rui and Lin, Junyang and Bai, Shuai and Li, Zhikang and Ma, Jianxin and Zhou, Chang and Zhou, Jingren and Yang, Hongxia},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), Computation and Language (cs.CL), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {OFA: Unifying Architectures, Tasks, and Modalities Through a Simple Sequence-to-Sequence Learning Framework},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {Creative Commons Attribution Share Alike 4.0 International}
}

@misc{unifiedio,
  doi = {10.48550/ARXIV.2206.08916},
  
  url = {https://arxiv.org/abs/2206.08916},
  
  author = {Lu, Jiasen and Clark, Christopher and Zellers, Rowan and Mottaghi, Roozbeh and Kembhavi, Aniruddha},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Unified-IO: A Unified Model for Vision, Language, and Multi-Modal Tasks},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {Creative Commons Attribution 4.0 International}
}

@misc{flamingo,
  doi = {10.48550/ARXIV.2204.14198},
  
  url = {https://arxiv.org/abs/2204.14198},
  
  author = {Alayrac, Jean-Baptiste and Donahue, Jeff and Luc, Pauline and Miech, Antoine and Barr, Iain and Hasson, Yana and Lenc, Karel and Mensch, Arthur and Millican, Katie and Reynolds, Malcolm and Ring, Roman and Rutherford, Eliza and Cabi, Serkan and Han, Tengda and Gong, Zhitao and Samangooei, Sina and Monteiro, Marianne and Menick, Jacob and Borgeaud, Sebastian and Brock, Andrew and Nematzadeh, Aida and Sharifzadeh, Sahand and Binkowski, Mikolaj and Barreira, Ricardo and Vinyals, Oriol and Zisserman, Andrew and Simonyan, Karen},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), Artificial Intelligence (cs.AI), Machine Learning (cs.LG), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Flamingo: a Visual Language Model for Few-Shot Learning},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}


@misc{pixel2seq,
  doi = {10.48550/ARXIV.2109.10852},
  
  url = {https://arxiv.org/abs/2109.10852},
  
  author = {Chen, Ting and Saxena, Saurabh and Li, Lala and Fleet, David J. and Hinton, Geoffrey},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), Artificial Intelligence (cs.AI), Computation and Language (cs.CL), Machine Learning (cs.LG), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Pix2seq: A Language Modeling Framework for Object Detection},
  
  publisher = {arXiv},
  
  year = {2021},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@misc{yan2020neural,
  doi = {10.48550/ARXIV.2001.02799},
  
  url = {https://arxiv.org/abs/2001.02799},
  
  author = {Yan, Xi and Acuna, David and Fidler, Sanja},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), Machine Learning (cs.LG), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Neural Data Server: A Large-Scale Search Engine for Transfer Learning Data},
  
  publisher = {arXiv},
  
  year = {2020},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@article{tanl,
  doi = {10.48550/ARXIV.2101.05779},
  
  url = {https://arxiv.org/abs/2101.05779},
  
  author = {Paolini, Giovanni and Athiwaratkun, Ben and Krone, Jason and Ma, Jie and Achille, Alessandro and Anubhai, Rishita and Santos, Cicero Nogueira dos and Xiang, Bing and Soatto, Stefano},
  
  keywords = {Machine Learning (cs.LG), Computation and Language (cs.CL), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Structured Prediction as Translation between Augmented Natural Languages},
  
  publisher = {arXiv},
  
  year = {2021},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@inproceedings{pseudo_labels,
  title={Pseudo-Label : The Simple and Efficient Semi-Supervised Learning Method for Deep Neural Networks},
  author={Dong-Hyun Lee},
  year={2013}
}

@misc{fixmatch,
  doi = {10.48550/ARXIV.2001.07685},
  
  url = {https://arxiv.org/abs/2001.07685},
  
  author = {Sohn, Kihyuk and Berthelot, David and Li, Chun-Liang and Zhang, Zizhao and Carlini, Nicholas and Cubuk, Ekin D. and Kurakin, Alex and Zhang, Han and Raffel, Colin},
  
  keywords = {Machine Learning (cs.LG), Computer Vision and Pattern Recognition (cs.CV), Machine Learning (stat.ML), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {FixMatch: Simplifying Semi-Supervised Learning with Consistency and Confidence},
  
  publisher = {arXiv},
  
  year = {2020},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}


@INPROCEEDINGS{open_set_DA,
  author={Busto, Pau Panareda and Gall, Juergen},
  booktitle={2017 IEEE International Conference on Computer Vision (ICCV)}, 
  title={Open Set Domain Adaptation}, 
  year={2017},
  volume={},
  number={},
  pages={754-763},
  doi={10.1109/ICCV.2017.88}}


@misc{open_set_DA_backpropagation,
  doi = {10.48550/ARXIV.1804.10427},
  
  url = {https://arxiv.org/abs/1804.10427},
  
  author = {Saito, Kuniaki and Yamamoto, Shohei and Ushiku, Yoshitaka and Harada, Tatsuya},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Open Set Domain Adaptation by Backpropagation},
  
  publisher = {arXiv},
  
  year = {2018},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@article{active_learning_survey,
  title={Active learning literature survey},
  author={Settles, Burr},
  year={2009},
  publisher={University of Wisconsin-Madison Department of Computer Sciences}
}

@misc{VOS,
  doi = {10.48550/ARXIV.2202.01197},
  
  url = {https://arxiv.org/abs/2202.01197},
  
  author = {Du, Xuefeng and Wang, Zhaoning and Cai, Mu and Li, Yixuan},
  
  keywords = {Machine Learning (cs.LG), Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {VOS: Learning What You Don't Know by Virtual Outlier Synthesis},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@misc{OOD_survey,
  doi = {10.48550/ARXIV.2110.11334},
  
  url = {https://arxiv.org/abs/2110.11334},
  
  author = {Yang, Jingkang and Zhou, Kaiyang and Li, Yixuan and Liu, Ziwei},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), Artificial Intelligence (cs.AI), Machine Learning (cs.LG), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Generalized Out-of-Distribution Detection: A Survey},
  
  publisher = {arXiv},
  
  year = {2021},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@misc{retrieval_language_model,
  doi = {10.48550/ARXIV.2102.02557},
  
  url = {https://arxiv.org/abs/2102.02557},
  
  author = {Yogatama, Dani and d'Autume, Cyprien de Masson and Kong, Lingpeng},
  
  keywords = {Computation and Language (cs.CL), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Adaptive Semiparametric Language Models},
  
  publisher = {arXiv},
  
  year = {2021},
  
  copyright = {Creative Commons Attribution 4.0 International}
}

@inproceedings{retrieval_NLP,
 author = {Lewis, Patrick and Perez, Ethan and Piktus, Aleksandra and Petroni, Fabio and Karpukhin, Vladimir and Goyal, Naman and K\"{u}ttler, Heinrich and Lewis, Mike and Yih, Wen-tau and Rockt\"{a}schel, Tim and Riedel, Sebastian and Kiela, Douwe},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {H. Larochelle and M. Ranzato and R. Hadsell and M.F. Balcan and H. Lin},
 pages = {9459--9474},
 publisher = {Curran Associates, Inc.},
 title = {Retrieval-Augmented Generation for Knowledge-Intensive NLP Tasks},
 url = {https://proceedings.neurips.cc/paper/2020/file/6b493230205f780e1bc26945df7481e5-Paper.pdf},
 volume = {33},
 year = {2020}
}

@article{faiss,
  title={Billion-scale similarity search with {GPUs}},
  author={Johnson, Jeff and Douze, Matthijs and J{\'e}gou, Herv{\'e}},
  journal={IEEE Transactions on Big Data},
  volume={7},
  number={3},
  pages={535--547},
  year={2019},
  publisher={IEEE}
}


@InProceedings{scann,
  title = 	 {Accelerating Large-Scale Inference with Anisotropic Vector Quantization},
  author =       {Guo, Ruiqi and Sun, Philip and Lindgren, Erik and Geng, Quan and Simcha, David and Chern, Felix and Kumar, Sanjiv},
  booktitle = 	 {Proceedings of the 37th International Conference on Machine Learning},
  pages = 	 {3887--3896},
  year = 	 {2020},
  editor = 	 {III, Hal Daumé and Singh, Aarti},
  volume = 	 {119},
  series = 	 {Proceedings of Machine Learning Research},
  month = 	 {13--18 Jul},
  publisher =    {PMLR},
  pdf = 	 {http://proceedings.mlr.press/v119/guo20h/guo20h.pdf},
  url = 	 {https://proceedings.mlr.press/v119/guo20h.html},
  abstract = 	 {Quantization based techniques are the current state-of-the-art for scaling maximum inner product search to massive databases. Traditional approaches to quantization aim to minimize the reconstruction error of the database points. Based on the observation that for a given query, the database points that have the largest inner products are more relevant, we develop a family of anisotropic quantization loss functions. Under natural statistical assumptions, we show that quantization with these loss functions leads to a new variant of vector quantization that more greatly penalizes the parallel component of a datapoint’s residual relative to its orthogonal component. The proposed approach, whose implementation is open-source, achieves state-of-the-art results on the public benchmarks available at ann-benchmarks.com.}
}


@misc{mixup,
  doi = {10.48550/ARXIV.1710.09412},
  
  url = {https://arxiv.org/abs/1710.09412},
  
  author = {Zhang, Hongyi and Cisse, Moustapha and Dauphin, Yann N. and Lopez-Paz, David},
  
  keywords = {Machine Learning (cs.LG), Machine Learning (stat.ML), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {mixup: Beyond Empirical Risk Minimization},
  
  publisher = {arXiv},
  
  year = {2017},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}


@misc{randaugment,
  doi = {10.48550/ARXIV.1909.13719},
  
  url = {https://arxiv.org/abs/1909.13719},
  
  author = {Cubuk, Ekin D. and Zoph, Barret and Shlens, Jonathon and Le, Quoc V.},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {RandAugment: Practical automated data augmentation with a reduced search space},
  
  publisher = {arXiv},
  
  year = {2019},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}


@misc{retrieval_prompt,
  doi = {10.48550/ARXIV.2205.14704},
  
  url = {https://arxiv.org/abs/2205.14704},
  
  author = {Chen, Xiang and Li, Lei and Zhang, Ningyu and Liang, Xiaozhuan and Deng, Shumin and Tan, Chuanqi and Huang, Fei and Si, Luo and Chen, Huajun},
  
  keywords = {Computation and Language (cs.CL), Artificial Intelligence (cs.AI), Information Retrieval (cs.IR), Machine Learning (cs.LG), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Decoupling Knowledge from Memorization: Retrieval-augmented Prompt Learning},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}


@misc{UDA_OD,
  doi = {10.48550/ARXIV.1803.03243},
  
  url = {https://arxiv.org/abs/1803.03243},
  
  author = {Chen, Yuhua and Li, Wen and Sakaridis, Christos and Dai, Dengxin and Van Gool, Luc},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Domain Adaptive Faster R-CNN for Object Detection in the Wild},
  
  publisher = {arXiv},
  
  year = {2018},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@misc{UDA_semantic_seg,
  doi = {10.48550/ARXIV.1802.10349},
  
  url = {https://arxiv.org/abs/1802.10349},
  
  author = {Tsai, Yi-Hsuan and Hung, Wei-Chih and Schulter, Samuel and Sohn, Kihyuk and Yang, Ming-Hsuan and Chandraker, Manmohan},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Learning to Adapt Structured Output Space for Semantic Segmentation},
  
  publisher = {arXiv},
  
  year = {2018},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@misc{UDA_MJ,
  doi = {10.48550/ARXIV.1502.02791},
  
  url = {https://arxiv.org/abs/1502.02791},
  
  author = {Long, Mingsheng and Cao, Yue and Wang, Jianmin and Jordan, Michael I.},
  
  keywords = {Machine Learning (cs.LG), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Learning Transferable Features with Deep Adaptation Networks},
  
  publisher = {arXiv},
  
  year = {2015},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@article{timm_repo,
  doi = {10.48550/ARXIV.2106.10270},
  
  url = {https://arxiv.org/abs/2106.10270},
  
  author = {Steiner, Andreas and Kolesnikov, Alexander and Zhai, Xiaohua and Wightman, Ross and Uszkoreit, Jakob and Beyer, Lucas},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), Artificial Intelligence (cs.AI), Machine Learning (cs.LG), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {How to train your ViT? Data, Augmentation, and Regularization in Vision Transformers},
  
  publisher = {arXiv},
  
  year = {2021},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}



@misc{quality_not_quantity_Nguyen,
      title={Quality Not Quantity: On the Interaction between Dataset Design and Robustness of CLIP}, 
      author={Thao Nguyen and Gabriel Ilharco and Mitchell Wortsman and Sewoong Oh and Ludwig Schmidt},
      year={2023},
      eprint={2208.05516},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}


@misc{attendandexcite2023chefer,
      title={Attend-and-Excite: Attention-Based Semantic Guidance for Text-to-Image Diffusion Models}, 
      author={Hila Chefer and Yuval Alaluf and Yael Vinker and Lior Wolf and Daniel Cohen-Or},
      year={2023},
      eprint={2301.13826},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}

@misc{layoutcontrol2023vedaldi,
      title={Training-Free Layout Control with Cross-Attention Guidance}, 
      author={Minghao Chen and Iro Laina and Andrea Vedaldi},
      year={2023},
      eprint={2304.03373},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}




@InProceedings{ddmps-sohl-dickstein15,
  title = 	 {Deep Unsupervised Learning using Nonequilibrium Thermodynamics},
  author = 	 {Sohl-Dickstein, Jascha and Weiss, Eric and Maheswaranathan, Niru and Ganguli, Surya},
  booktitle = 	 {Proceedings of the 32nd International Conference on Machine Learning},
  pages = 	 {2256--2265},
  year = 	 {2015},
  editor = 	 {Bach, Francis and Blei, David},
  volume = 	 {37},
  series = 	 {Proceedings of Machine Learning Research},
  address = 	 {Lille, France},
  month = 	 {07--09 Jul},
  publisher =    {PMLR},
  pdf = 	 {http://proceedings.mlr.press/v37/sohl-dickstein15.pdf},
  url = 	 {https://proceedings.mlr.press/v37/sohl-dickstein15.html},
  abstract = 	 {A central problem in machine learning involves modeling complex data-sets using highly flexible families of probability distributions in which learning, sampling, inference, and evaluation are still analytically or computationally tractable. Here, we develop an approach that simultaneously achieves both flexibility and tractability. The essential idea, inspired by non-equilibrium statistical physics, is to systematically and slowly destroy structure in a data distribution through an iterative forward diffusion process. We then learn a reverse diffusion process that restores structure in data, yielding a highly flexible and tractable generative model of the data. This approach allows us to rapidly learn, sample from, and evaluate probabilities in deep generative models with thousands of layers or time steps, as well as to compute conditional and posterior probabilities under the learned model. We additionally release an open source reference implementation of the algorithm.}
}

@article{score_based_generative_models_Ermon19,
  author       = {Yang Song and
                  Stefano Ermon},
  title        = {Generative Modeling by Estimating Gradients of the Data Distribution},
  journal      = {CoRR},
  volume       = {abs/1907.05600},
  year         = {2019},
  url          = {http://arxiv.org/abs/1907.05600},
  eprinttype    = {arXiv},
  eprint       = {1907.05600},
  timestamp    = {Thu, 01 Oct 2020 17:52:46 +0200},
  biburl       = {https://dblp.org/rec/journals/corr/abs-1907-05600.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{ddim_ermon20,
  author       = {Jiaming Song and
                  Chenlin Meng and
                  Stefano Ermon},
  title        = {Denoising Diffusion Implicit Models},
  journal      = {CoRR},
  volume       = {abs/2010.02502},
  year         = {2020},
  url          = {https://arxiv.org/abs/2010.02502},
  eprinttype    = {arXiv},
  eprint       = {2010.02502},
  timestamp    = {Mon, 12 Oct 2020 17:53:10 +0200},
  biburl       = {https://dblp.org/rec/journals/corr/abs-2010-02502.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{stable_diffusion_Rombach_21,
  author       = {Robin Rombach and
                  Andreas Blattmann and
                  Dominik Lorenz and
                  Patrick Esser and
                  Bj{\"{o}}rn Ommer},
  title        = {High-Resolution Image Synthesis with Latent Diffusion Models},
  journal      = {CoRR},
  volume       = {abs/2112.10752},
  year         = {2021},
  url          = {https://arxiv.org/abs/2112.10752},
  eprinttype    = {arXiv},
  eprint       = {2112.10752},
  timestamp    = {Tue, 04 Jan 2022 15:59:27 +0100},
  biburl       = {https://dblp.org/rec/journals/corr/abs-2112-10752.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}


@article{controlnets_zhang23,
  title={Adding conditional control to text-to-image diffusion models},
  author={Zhang, Lvmin and Agrawala, Maneesh},
  journal={arXiv preprint arXiv:2302.05543},
  year={2023}
}

@article{dd_restoration_models_Ermon_22,
  title={Denoising diffusion restoration models},
  author={Kawar, Bahjat and Elad, Michael and Ermon, Stefano and Song, Jiaming},
  journal={arXiv preprint arXiv:2201.11793},
  year={2022}
}

@inproceedings{
pseudoinverseguided_song_23,
title={Pseudoinverse-Guided Diffusion Models for Inverse Problems},
author={Jiaming Song and Arash Vahdat and Morteza Mardani and Jan Kautz},
booktitle={International Conference on Learning Representations},
year={2023},
url={https://openreview.net/forum?id=9_gsMA8MRKQ}
}

@article{classifier_guidance_21,
  author       = {Prafulla Dhariwal and
                  Alex Nichol},
  title        = {Diffusion Models Beat GANs on Image Synthesis},
  journal      = {CoRR},
  volume       = {abs/2105.05233},
  year         = {2021},
  url          = {https://arxiv.org/abs/2105.05233},
  eprinttype    = {arXiv},
  eprint       = {2105.05233},
  timestamp    = {Fri, 14 May 2021 12:13:30 +0200},
  biburl       = {https://dblp.org/rec/journals/corr/abs-2105-05233.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{compositional_visual_generation_tenenbaum_22,
  title={Compositional visual generation with composable diffusion models},
  author={Liu, Nan and Li, Shuang and Du, Yilun and Torralba, Antonio and Tenenbaum, Joshua B},
  booktitle={Computer Vision--ECCV 2022: 17th European Conference, Tel Aviv, Israel, October 23--27, 2022, Proceedings, Part XVII},
  pages={423--439},
  year={2022},
  organization={Springer}
}

@article{diffusion_posterior_sampling_22,
  title={Diffusion posterior sampling for general noisy inverse problems},
  author={Chung, Hyungjin and Kim, Jeongsol and Mccann, Michael T and Klasky, Marc L and Ye, Jong Chul},
  journal={arXiv preprint arXiv:2209.14687},
  year={2022}
}

@article{prompt2prompt_cross_attention_control,
  title={Prompt-to-prompt image editing with cross attention control},
  author={Hertz, Amir and Mokady, Ron and Tenenbaum, Jay and Aberman, Kfir and Pritch, Yael and Cohen-Or, Daniel},
  journal={arXiv preprint arXiv:2208.01626},
  year={2022}
}


@article{lindquist1985forward,
  title={Forward and backward semimartingale models for Gaussian processes with stationary increments},
  author={Lindquist, Anders and Picci, Giorgio},
  journal={Stochastics: An International Journal of Probability and Stochastic Processes},
  volume={15},
  number={1},
  pages={1--50},
  year={1985},
  publisher={Taylor \& Francis}
}

@article{lindquist1979stochastic,
  title={On the stochastic realization problem},
  author={Lindquist, Anders and Picci, Giorgio},
  journal={SIAM Journal on Control and Optimization},
  volume={17},
  number={3},
  pages={365--389},
  year={1979},
  publisher={SIAM}
}

@article{anderson1982reverse,
  title={Reverse-time diffusion equation models},
  author={Anderson, Brian DO},
  journal={Stochastic Processes and their Applications},
  volume={12},
  number={3},
  pages={313--326},
  year={1982},
  publisher={Elsevier}
}

@book{nelson1967dynamical,
  title={Dynamical theories of Brownian motion},
  author={Nelson, Edward},
  year={1967},
  publisher={Princeton university press}
}


@article{rameshHierarchicalTextConditionalImage2022,
	title = {Hierarchical {Text}-{Conditional} {Image} {Generation} with {CLIP} {Latents}},
	url = {http://arxiv.org/abs/2204.06125},
	abstract = {Contrastive models like CLIP have been shown to learn robust representations of images that capture both semantics and style. To leverage these representations for image generation, we propose a two-stage model: a prior that generates a CLIP image embedding given a text caption, and a decoder that generates an image conditioned on the image embedding. We show that explicitly generating image representations improves image diversity with minimal loss in photorealism and caption similarity. Our decoders conditioned on image representations can also produce variations of an image that preserve both its semantics and style, while varying the non-essential details absent from the image representation. Moreover, the joint embedding space of CLIP enables language-guided image manipulations in a zero-shot fashion. We use diffusion models for the decoder and experiment with both autoregressive and diffusion models for the prior, ﬁnding that the latter are computationally more efﬁcient and produce higher-quality samples.},
	language = {en},
	urldate = {2022-04-29},
	journal = {arXiv:2204.06125 [cs]},
	author = {Ramesh, Aditya and Dhariwal, Prafulla and Nichol, Alex and Chu, Casey and Chen, Mark},
	month = apr,
	year = {2022},
	note = {arXiv: 2204.06125},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
	file = {Ramesh et al. - 2022 - Hierarchical Text-Conditional Image Generation wit.pdf:/Users/mttrager/Zotero/storage/LN3DBQDN/Ramesh et al. - 2022 - Hierarchical Text-Conditional Image Generation wit.pdf:application/pdf},
}



@misc{sahariaPhotorealisticTexttoImageDiffusion2022,
	title = {Photorealistic {Text}-to-{Image} {Diffusion} {Models} with {Deep} {Language} {Understanding}},
	url = {http://arxiv.org/abs/2205.11487},
	abstract = {We present Imagen, a text-to-image diffusion model with an unprecedented degree of photorealism and a deep level of language understanding. Imagen builds on the power of large transformer language models in understanding text and hinges on the strength of diffusion models in high-ﬁdelity image generation. Our key discovery is that generic large language models (e.g. T5), pretrained on text-only corpora, are surprisingly effective at encoding text for image synthesis: increasing the size of the language model in Imagen boosts both sample ﬁdelity and imagetext alignment much more than increasing the size of the image diffusion model. Imagen achieves a new state-of-the-art FID score of 7.27 on the COCO dataset, without ever training on COCO, and human raters ﬁnd Imagen samples to be on par with the COCO data itself in image-text alignment. To assess text-to-image models in greater depth, we introduce DrawBench, a comprehensive and challenging benchmark for text-to-image models. With DrawBench, we compare Imagen with recent methods including VQ-GAN+CLIP, Latent Diffusion Models, GLIDE and DALL-E 2, and ﬁnd that human raters prefer Imagen over other models in side-byside comparisons, both in terms of sample quality and image-text alignment. See imagen.research.google for an overview of the results.},
	language = {en},
	urldate = {2022-05-25},
	publisher = {arXiv},
	author = {Saharia, Chitwan and Chan, William and Saxena, Saurabh and Li, Lala and Whang, Jay and Denton, Emily and Ghasemipour, Seyed Kamyar Seyed and Ayan, Burcu Karagol and Mahdavi, S. Sara and Lopes, Rapha Gontijo and Salimans, Tim and Ho, Jonathan and Fleet, David J. and Norouzi, Mohammad},
	month = may,
	year = {2022},
	note = {Number: arXiv:2205.11487
arXiv:2205.11487 [cs]},
	keywords = {Computer Science - Machine Learning, Computer Science - Computer Vision and Pattern Recognition},
	file = {Saharia et al. - 2022 - Photorealistic Text-to-Image Diffusion Models with.pdf:/Users/mttrager/Zotero/storage/E67SLJHG/Saharia et al. - 2022 - Photorealistic Text-to-Image Diffusion Models with.pdf:application/pdf},
}


@article{radfordLearningTransferableVisual2021,
	title = {Learning {Transferable} {Visual} {Models} {From} {Natural} {Language} {Supervision}},
	url = {http://arxiv.org/abs/2103.00020},
	abstract = {State-of-the-art computer vision systems are trained to predict a ﬁxed set of predetermined object categories. This restricted form of supervision limits their generality and usability since additional labeled data is needed to specify any other visual concept. Learning directly from raw text about images is a promising alternative which leverages a much broader source of supervision. We demonstrate that the simple pre-training task of predicting which caption goes with which image is an efﬁcient and scalable way to learn SOTA image representations from scratch on a dataset of 400 million (image, text) pairs collected from the internet. After pre-training, natural language is used to reference learned visual concepts (or describe new ones) enabling zero-shot transfer of the model to downstream tasks. We study the performance of this approach by benchmarking on over 30 different existing computer vision datasets, spanning tasks such as OCR, action recognition in videos, geo-localization, and many types of ﬁne-grained object classiﬁcation. The model transfers non-trivially to most tasks and is often competitive with a fully supervised baseline without the need for any dataset speciﬁc training. For instance, we match the accuracy of the original ResNet-50 on ImageNet zero-shot without needing to use any of the 1.28 million training examples it was trained on. We release our code and pre-trained model weights at https://github.com/OpenAI/CLIP.},
	language = {en},
	urldate = {2022-04-29},
	journal = {arXiv:2103.00020 [cs]},
	author = {Radford, Alec and Kim, Jong Wook and Hallacy, Chris and Ramesh, Aditya and Goh, Gabriel and Agarwal, Sandhini and Sastry, Girish and Askell, Amanda and Mishkin, Pamela and Clark, Jack and Krueger, Gretchen and Sutskever, Ilya},
	month = feb,
	year = {2021},
	note = {arXiv: 2103.00020},
	keywords = {Computer Science - Machine Learning, Computer Science - Computer Vision and Pattern Recognition},
	file = {Radford et al. - 2021 - Learning Transferable Visual Models From Natural L.pdf:/Users/mttrager/Zotero/storage/H5KGXF33/Radford et al. - 2021 - Learning Transferable Visual Models From Natural L.pdf:application/pdf},
}



@misc{liptonPreciseRecoveryLatent2017,
	title = {Precise {Recovery} of {Latent} {Vectors} from {Generative} {Adversarial} {Networks}},
	url = {http://arxiv.org/abs/1702.04782},
	abstract = {Generative adversarial networks (GANs) transform latent vectors into visually plausible images. It is generally thought that the original GAN formulation gives no out-of-the-box method to reverse the mapping, projecting images back into latent space. We introduce a simple, gradient-based technique called stochastic clipping. In experiments, for images generated by the GAN, we precisely recover their latent vector pre-images 100\% of the time. Additional experiments demonstrate that this method is robust to noise. Finally, we show that even for unseen images, our method appears to recover unique encodings.},
	language = {en},
	urldate = {2023-05-17},
	publisher = {arXiv},
	author = {Lipton, Zachary C. and Tripathi, Subarna},
	month = feb,
	year = {2017},
	note = {arXiv:1702.04782 [cs, stat]},
	keywords = {Computer Science - Machine Learning, Computer Science - Neural and Evolutionary Computing, Statistics - Machine Learning},
	file = {Lipton and Tripathi - 2017 - Precise Recovery of Latent Vectors from Generative.pdf:/Users/mttrager/Zotero/storage/HXJIYZ3B/Lipton and Tripathi - 2017 - Precise Recovery of Latent Vectors from Generative.pdf:application/pdf},
}



@misc{abdalImage2StyleGANHowEmbed2019,
	title = {{Image2StyleGAN}: {How} to {Embed} {Images} {Into} the {StyleGAN} {Latent} {Space}?},
	shorttitle = {{Image2StyleGAN}},
	url = {http://arxiv.org/abs/1904.03189},
	abstract = {We propose an efﬁcient algorithm to embed a given image into the latent space of StyleGAN. This embedding enables semantic image editing operations that can be applied to existing photographs. Taking the StyleGAN trained on the FFHQ dataset as an example, we show results for image morphing, style transfer, and expression transfer. Studying the results of the embedding algorithm provides valuable insights into the structure of the StyleGAN latent space. We propose a set of experiments to test what class of images can be embedded, how they are embedded, what latent space is suitable for embedding, and if the embedding is semantically meaningful.},
	language = {en},
	urldate = {2023-05-17},
	publisher = {arXiv},
	author = {Abdal, Rameen and Qin, Yipeng and Wonka, Peter},
	month = sep,
	year = {2019},
	note = {arXiv:1904.03189 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
	annote = {Comment: Accepted for oral presentation at ICCV 2019, "For videos visit https://youtu.be/RnTXLXw9o\_I , https://youtu.be/zJoYY2eHAF0 and https://youtu.be/bA893L-PjbI"},
	file = {Abdal et al. - 2019 - Image2StyleGAN How to Embed Images Into the Style.pdf:/Users/mttrager/Zotero/storage/MTWKZT6Z/Abdal et al. - 2019 - Image2StyleGAN How to Embed Images Into the Style.pdf:application/pdf},
}


@misc{creswellInvertingGeneratorGenerative2016,
	title = {Inverting {The} {Generator} {Of} {A} {Generative} {Adversarial} {Network}},
	url = {http://arxiv.org/abs/1611.05644},
	abstract = {Generative adversarial networks (GANs) learn to synthesise new samples from a high-dimensional distribution by passing samples drawn from a latent space through a generative network. When the high-dimensional distribution describes images of a particular data set, the network should learn to generate visually similar image samples for latent variables that are close to each other in the latent space. For tasks such as image retrieval and image classiﬁcation, it may be useful to exploit the arrangement of the latent space by projecting images into it, and using this as a representation for discriminative tasks. GANs often consist of multiple layers of non-linear computations, making them very difﬁcult to invert. This paper introduces techniques for projecting image samples into the latent space using any pre-trained GAN, provided that the computational graph is available. We evaluate these techniques on both MNIST digits and Omniglot handwritten characters. In the case of MNIST digits, we show that projections into the latent space maintain information about the style and the identity of the digit. In the case of Omniglot characters, we show that even characters from alphabets that have not been seen during training may be projected well into the latent space; this suggests that this approach may have applications in one-shot learning.},
	language = {en},
	urldate = {2023-05-17},
	publisher = {arXiv},
	author = {Creswell, Antonia and Bharath, Anil Anthony},
	month = nov,
	year = {2016},
	note = {arXiv:1611.05644 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition, Computer Science - Machine Learning},
	annote = {Comment: Accepted at NIPS 2016 Workshop on Adversarial Training},
	file = {Creswell and Bharath - 2016 - Inverting The Generator Of A Generative Adversaria.pdf:/Users/mttrager/Zotero/storage/GNKTJ6IH/Creswell and Bharath - 2016 - Inverting The Generator Of A Generative Adversaria.pdf:application/pdf},
}


@misc{ruizDreamBoothFineTuning2022,
	title = {{DreamBooth}: {Fine} {Tuning} {Text}-to-{Image} {Diffusion} {Models} for {Subject}-{Driven} {Generation}},
	shorttitle = {{DreamBooth}},
	url = {http://arxiv.org/abs/2208.12242},
	abstract = {Large text-to-image models achieved a remarkable leap in the evolution of AI, enabling high-quality and diverse synthesis of images from a given text prompt. However, these models lack the ability to mimic the appearance of subjects in a given reference set and synthesize novel renditions of them in different contexts. In this work, we present a new approach for "personalization" of text-to-image diffusion models (specializing them to users' needs). Given as input just a few images of a subject, we fine-tune a pretrained text-to-image model (Imagen, although our method is not limited to a specific model) such that it learns to bind a unique identifier with that specific subject. Once the subject is embedded in the output domain of the model, the unique identifier can then be used to synthesize fully-novel photorealistic images of the subject contextualized in different scenes. By leveraging the semantic prior embedded in the model with a new autogenous class-specific prior preservation loss, our technique enables synthesizing the subject in diverse scenes, poses, views, and lighting conditions that do not appear in the reference images. We apply our technique to several previously-unassailable tasks, including subject recontextualization, text-guided view synthesis, appearance modification, and artistic rendering (all while preserving the subject's key features). Project page: https://dreambooth.github.io/},
	language = {en},
	urldate = {2022-12-07},
	publisher = {arXiv},
	author = {Ruiz, Nataniel and Li, Yuanzhen and Jampani, Varun and Pritch, Yael and Rubinstein, Michael and Aberman, Kfir},
	month = aug,
	year = {2022},
	note = {arXiv:2208.12242 [cs]},
	keywords = {Computer Science - Machine Learning, Computer Science - Computer Vision and Pattern Recognition, Computer Science - Graphics},
	annote = {Comment: Project page: https://dreambooth.github.io/},
	file = {Ruiz et al. - 2022 - DreamBooth Fine Tuning Text-to-Image Diffusion Mo.pdf:/Users/mttrager/Zotero/storage/IZAWGVXS/Ruiz et al. - 2022 - DreamBooth Fine Tuning Text-to-Image Diffusion Mo.pdf:application/pdf},
}

@misc{mokadyNulltextInversionEditing2022,
	title = {Null-text {Inversion} for {Editing} {Real} {Images} using {Guided} {Diffusion} {Models}},
	url = {http://arxiv.org/abs/2211.09794},
	abstract = {Recent text-guided diffusion models provide powerful image generation capabilities. Currently, a massive effort is given to enable the modiﬁcation of these images using text only as means to offer intuitive and versatile editing. To edit a real image using these state-of-the-art tools, one must ﬁrst invert the image with a meaningful text prompt into the pretrained model’s domain. In this paper, we introduce an accurate inversion technique and thus facilitate an intuitive text-based modiﬁcation of the image. Our proposed inversion consists of two novel key components: (i) Pivotal inversion for diffusion models. While current methods aim at mapping random noise samples to a single input image, we use a single pivotal noise vector for each timestamp and optimize around it. We demonstrate that a direct inversion is inadequate on its own, but does provide a good anchor for our optimization. (ii) null-text optimization, where we only modify the unconditional textual embedding that is used for classiﬁer-free guidance, rather than the input text embedding. This allows for keeping both the model weights and the conditional embedding intact and hence enables applying prompt-based editing while avoiding the cumbersome tuning of the model’s weights. Our null-text inversion, based on the publicly available Stable Diffusion model, is extensively evaluated on a variety of images and prompt editing, showing high-ﬁdelity editing of real images.},
	language = {en},
	urldate = {2023-05-17},
	publisher = {arXiv},
	author = {Mokady, Ron and Hertz, Amir and Aberman, Kfir and Pritch, Yael and Cohen-Or, Daniel},
	month = nov,
	year = {2022},
	note = {arXiv:2211.09794 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
	file = {Mokady et al. - 2022 - Null-text Inversion for Editing Real Images using .pdf:/Users/mttrager/Zotero/storage/UYH574V4/Mokady et al. - 2022 - Null-text Inversion for Editing Real Images using .pdf:application/pdf},
}




@misc{dongPromptTuningInversion2023,
	title = {Prompt {Tuning} {Inversion} for {Text}-{Driven} {Image} {Editing} {Using} {Diffusion} {Models}},
	url = {http://arxiv.org/abs/2305.04441},
	abstract = {Recently large-scale language-image models (e.g., textguided diffusion models) have considerably improved the image generation capabilities to generate photorealistic images in various domains. Based on this success, current image editing methods use texts to achieve intuitive and versatile modiﬁcation of images. To edit a real image using diffusion models, one must ﬁrst invert the image to a noisy latent from which an edited image is sampled with a target text prompt. However, most methods lack one of the following: user-friendliness (e.g., additional masks or precise descriptions of the input image are required), generalization to larger domains, or high ﬁdelity to the input image. In this paper, we design an accurate and quick inversion technique, Prompt Tuning Inversion, for text-driven image editing. Speciﬁcally, our proposed editing method consists of a reconstruction stage and an editing stage. In the ﬁrst stage, we encode the information of the input image into a learnable conditional embedding via Prompt Tuning Inversion. In the second stage, we apply classiﬁer-free guidance to sample the edited image, where the conditional embedding is calculated by linearly interpolating between the target embedding and the optimized one obtained in the ﬁrst stage. This technique ensures a superior trade-off between editability and high ﬁdelity to the input image of our method. For example, we can change the color of a speciﬁc object while preserving its original shape and background under the guidance of only a target text prompt. Extensive experiments on ImageNet demonstrate the superior editing performance of our method compared to the state-of-the-art baselines.},
	language = {en},
	urldate = {2023-05-17},
	publisher = {arXiv},
	author = {Dong, Wenkai and Xue, Song and Duan, Xiaoyue and Han, Shumin},
	month = may,
	year = {2023},
	note = {arXiv:2305.04441 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
	file = {Dong et al. - 2023 - Prompt Tuning Inversion for Text-Driven Image Edit.pdf:/Users/mttrager/Zotero/storage/NFWQDEPA/Dong et al. - 2023 - Prompt Tuning Inversion for Text-Driven Image Edit.pdf:application/pdf},
}



@article{liuPretrainPromptPredict2021,
	title = {Pre-train, {Prompt}, and {Predict}: {A} {Systematic} {Survey} of {Prompting} {Methods} in {Natural} {Language} {Processing}},
	shorttitle = {Pre-train, {Prompt}, and {Predict}},
	url = {http://arxiv.org/abs/2107.13586},
	abstract = {This paper surveys and organizes research works in a new paradigm in natural language processing, which we dub "prompt-based learning". Unlike traditional supervised learning, which trains a model to take in an input x and predict an output y as P(y{\textbar}x), prompt-based learning is based on language models that model the probability of text directly. To use these models to perform prediction tasks, the original input x is modified using a template into a textual string prompt x' that has some unfilled slots, and then the language model is used to probabilistically fill the unfilled information to obtain a final string x, from which the final output y can be derived. This framework is powerful and attractive for a number of reasons: it allows the language model to be pre-trained on massive amounts of raw text, and by defining a new prompting function the model is able to perform few-shot or even zero-shot learning, adapting to new scenarios with few or no labeled data. In this paper we introduce the basics of this promising paradigm, describe a unified set of mathematical notations that can cover a wide variety of existing work, and organize existing work along several dimensions, e.g.the choice of pre-trained models, prompts, and tuning strategies. To make the field more accessible to interested beginners, we not only make a systematic review of existing works and a highly structured typology of prompt-based concepts, but also release other resources, e.g., a website http://pretrain.nlpedia.ai/ including constantly-updated survey, and paperlist.},
	language = {en},
	urldate = {2021-09-08},
	journal = {arXiv:2107.13586 [cs]},
	author = {Liu, Pengfei and Yuan, Weizhe and Fu, Jinlan and Jiang, Zhengbao and Hayashi, Hiroaki and Neubig, Graham},
	month = jul,
	year = {2021},
	note = {arXiv: 2107.13586},
	keywords = {Computer Science - Machine Learning, Computer Science - Artificial Intelligence, Computer Science - Computation and Language},
	annote = {Comment: Website: http://pretrain.nlpedia.ai/},
	file = {Liu et al. - 2021 - Pre-train, Prompt, and Predict A Systematic Surve.pdf:/Users/mttrager/Zotero/storage/CSX45LNE/Liu et al. - 2021 - Pre-train, Prompt, and Predict A Systematic Surve.pdf:application/pdf},
}

@InProceedings{Naeem_2021_CVPR,
    author    = {Naeem, Muhammad Ferjad and Xian, Yongqin and Tombari, Federico and Akata, Zeynep},
    title     = {Learning Graph Embeddings for Compositional Zero-Shot Learning},
    booktitle = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
    month     = {June},
    year      = {2021},
    pages     = {953-962}
}

@article{ge2019deepfashion2,
  abstract = {Understanding fashion images has been advanced by benchmarks with rich
annotations such as DeepFashion, whose labels include clothing categories,
landmarks, and consumer-commercial image pairs. However, DeepFashion has
nonnegligible issues such as single clothing-item per image, sparse landmarks
(4~8 only), and no per-pixel masks, making it had significant gap from
real-world scenarios. We fill in the gap by presenting DeepFashion2 to address
these issues. It is a versatile benchmark of four tasks including clothes
detection, pose estimation, segmentation, and retrieval. It has 801K clothing
items where each item has rich annotations such as style, scale, viewpoint,
occlusion, bounding box, dense landmarks and masks. There are also 873K
Commercial-Consumer clothes pairs. A strong baseline is proposed, called Match
R-CNN, which builds upon Mask R-CNN to solve the above four tasks in an
end-to-end manner. Extensive evaluations are conducted with different
criterions in DeepFashion2.},
  added-at = {2019-03-09T01:56:57.000+0100},
  author = {Ge, Yuying and Zhang, Ruimao and Wu, Lingyun and Wang, Xiaogang and Tang, Xiaoou and Luo, Ping},
  biburl = {https://www.bibsonomy.org/bibtex/2b3510872d1f5220259cf26b2c2fe2e47/kirk86},
  description = {[1901.07973] DeepFashion2: A Versatile Benchmark for Detection, Pose Estimation, Segmentation and Re-Identification of Clothing Images},
  interhash = {651256a779bf88278846826613bb6a1e},
  intrahash = {b3510872d1f5220259cf26b2c2fe2e47},
  keywords = {benchmarks deep-learning},
  note = {cite arxiv:1901.07973},
  timestamp = {2019-03-09T01:56:57.000+0100},
  title = {DeepFashion2: A Versatile Benchmark for Detection, Pose Estimation,
  Segmentation and Re-Identification of Clothing Images},
  url = {http://arxiv.org/abs/1901.07973},
  year = 2019
}




@incollection{cohenThisMyUnicorn2022a,
	address = {Cham},
	title = {“{This} {Is} {My} {Unicorn}, {Fluffy}”: {Personalizing} {Frozen} {Vision}-{Language} {Representations}},
	volume = {13680},
	isbn = {978-3-031-20043-4 978-3-031-20044-1},
	shorttitle = {“{This} {Is} {My} {Unicorn}, {Fluffy}”},
	url = {https://link.springer.com/10.1007/978-3-031-20044-1_32},
	abstract = {Large Vision \& Language models pretrained on web-scale data provide representations that are invaluable for numerous V\&L problems. However, it is unclear how they can be extended to reason about user-specific visual concepts in unstructured language. This problem arises in multiple domains, from personalized image retrieval to personalized interaction with smart devices. We introduce a new learning setup called Personalized Vision \& Language (PerVL) with two new benchmark datasets for retrieving and segmenting user-specific (“personalized”) concepts “in the wild”. In PerVL, one should learn personalized concepts (1) independently of the downstream task (2) allowing a pretrained model to reason about them with free language, and (3) without providing personalized negative examples. We propose an architecture for solving PerVL that operates by expanding the input vocabulary of a pretrained model with new word embeddings for the personalized concepts. The model can then simply employ them as part of a sentence. We demonstrate that our approach learns personalized visual concepts from a few examples and effectively applies them in image retrieval and semantic segmentation using rich textual queries. For example the model improves MRR by 51.1\% (28.4\% vs 18.8\%) compared to the strongest baseline.},
	language = {en},
	urldate = {2023-02-24},
	booktitle = {Computer {Vision} – {ECCV} 2022},
	publisher = {Springer Nature Switzerland},
	author = {Cohen, Niv and Gal, Rinon and Meirom, Eli A. and Chechik, Gal and Atzmon, Yuval},
	editor = {Avidan, Shai and Brostow, Gabriel and Cissé, Moustapha and Farinella, Giovanni Maria and Hassner, Tal},
	year = {2022},
	doi = {10.1007/978-3-031-20044-1_32},
	note = {Series Title: Lecture Notes in Computer Science},
	pages = {558--577},
	file = {Cohen et al. - 2022 - “This Is My Unicorn, Fluffy” Personalizing Frozen.pdf:/Users/mttrager/Zotero/storage/5N2UU5DL/Cohen et al. - 2022 - “This Is My Unicorn, Fluffy” Personalizing Frozen.pdf:application/pdf},
}



@misc{saitoPic2WordMappingPictures2023,
	title = {{Pic2Word}: {Mapping} {Pictures} to {Words} for {Zero}-shot {Composed} {Image} {Retrieval}},
	shorttitle = {{Pic2Word}},
	url = {http://arxiv.org/abs/2302.03084},
	abstract = {In Composed Image Retrieval (CIR), a user combines a query image with text to describe their intended target. Existing methods rely on supervised learning of CIR models using labeled triplets consisting of the query image, text specification, and the target image. Labeling such triplets is expensive and hinders broad applicability of CIR. In this work, we propose to study an important task, Zero-Shot Composed Image Retrieval (ZS-CIR), whose goal is to build a CIR model without requiring labeled triplets for training. To this end, we propose a novel method, called Pic2Word, that requires only weakly labeled image-caption pairs and unlabeled image datasets to train. Unlike existing supervised CIR models, our model trained on weakly labeled or unlabeled datasets shows strong generalization across diverse ZS-CIR tasks, e.g., attribute editing, object composition, and domain conversion. Our approach outperforms several supervised CIR methods on the common CIR benchmark, CIRR and Fashion-IQ. Code will be made publicly available at https://github.com/google-research/composed\_image\_retrieval.},
	language = {en},
	urldate = {2023-03-14},
	publisher = {arXiv},
	author = {Saito, Kuniaki and Sohn, Kihyuk and Zhang, Xiang and Li, Chun-Liang and Lee, Chen-Yu and Saenko, Kate and Pfister, Tomas},
	month = feb,
	year = {2023},
	note = {arXiv:2302.03084 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
	file = {Saito et al. - 2023 - Pic2Word Mapping Pictures to Words for Zero-shot .pdf:/Users/mttrager/Zotero/storage/NQZ6BSSM/Saito et al. - 2023 - Pic2Word Mapping Pictures to Words for Zero-shot .pdf:application/pdf},
}




@misc{jiaVisualPromptTuning2022,
	title = {Visual {Prompt} {Tuning}},
	url = {http://arxiv.org/abs/2203.12119},
	abstract = {The current modus operandi in adapting pre-trained models involves updating all the backbone parameters, i.e., full fine-tuning. This paper introduces Visual Prompt Tuning (VPT) as an efficient and effective alternative to full fine-tuning for large-scale Transformer models in vision. Taking inspiration from recent advances in efficiently tuning large language models, VPT introduces only a small amount (less than 1\% of model parameters) of trainable parameters in the input space while keeping the model backbone frozen. Via extensive experiments on a wide variety of downstream recognition tasks, we show that VPT achieves significant performance gains compared to other parameter efficient tuning protocols. Most importantly, VPT even outperforms full fine-tuning in many cases across model capacities and training data scales, while reducing per-task storage cost. Code is available at github.com/kmnp/vpt.},
	language = {en},
	urldate = {2023-05-17},
	publisher = {arXiv},
	author = {Jia, Menglin and Tang, Luming and Chen, Bor-Chun and Cardie, Claire and Belongie, Serge and Hariharan, Bharath and Lim, Ser-Nam},
	month = jul,
	year = {2022},
	note = {arXiv:2203.12119 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
	annote = {Comment: ECCV2022},
	file = {Jia et al. - 2022 - Visual Prompt Tuning.pdf:/Users/mttrager/Zotero/storage/HFKH6N22/Jia et al. - 2022 - Visual Prompt Tuning.pdf:application/pdf},
}


@inproceedings{lester-etal-2021-power,
    title = "The Power of Scale for Parameter-Efficient Prompt Tuning",
    author = "Lester, Brian  and
      Al-Rfou, Rami  and
      Constant, Noah",
    booktitle = "Proceedings of the 2021 Conference on Empirical Methods in Natural Language Processing",
    month = nov,
    year = "2021",
    address = "Online and Punta Cana, Dominican Republic",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2021.emnlp-main.243",
    doi = "10.18653/v1/2021.emnlp-main.243",
    pages = "3045--3059",
    abstract = "In this work, we explore {``}prompt tuning,{''} a simple yet effective mechanism for learning {``}soft prompts{''} to condition frozen language models to perform specific downstream tasks. Unlike the discrete text prompts used by GPT-3, soft prompts are learned through backpropagation and can be tuned to incorporate signals from any number of labeled examples. Our end-to-end learned approach outperforms GPT-3{'}s few-shot learning by a large margin. More remarkably, through ablations on model size using T5, we show that prompt tuning becomes more competitive with scale: as models exceed billions of parameters, our method {``}closes the gap{''} and matches the strong performance of model tuning (where all model weights are tuned). This finding is especially relevant because large models are costly to share and serve and the ability to reuse one frozen model for multiple downstream tasks can ease this burden. Our method can be seen as a simplification of the recently proposed {``}prefix tuning{''} of Li and Liang (2021) and we provide a comparison to this and other similar approaches. Finally, we show that conditioning a frozen model with soft prompts confers benefits in robustness to domain transfer and enables efficient {``}prompt ensembling.{''} We release code and model checkpoints to reproduce our experiments.",
}


@misc{nayakLearningComposeSoft2022,
	title = {Learning to {Compose} {Soft} {Prompts} for {Compositional} {Zero}-{Shot} {Learning}},
	url = {http://arxiv.org/abs/2204.03574},
	abstract = {We introduce compositional soft prompting (CSP), a parameter-efﬁcient learning technique to improve the zero-shot compositionality of large-scale pretrained vision-language models (VLMs) without the overhead of ﬁne-tuning the entire model. VLMs can represent arbitrary classes as natural language prompts in their ﬂexible text encoders but they underperform state-of-the-art methods on compositional zero-shot benchmark tasks. To improve VLMs, we propose a novel form of soft prompting. We treat the attributes and objects that are composed to deﬁne classes as learnable tokens of vocabulary and tune them on multiple prompt compositions. During inference, we recompose the learned attribute-object vocabulary in new combinations and show that CSP outperforms the original VLM on benchmark datasets by an average of 14.7 percentage points of accuracy. CSP also achieves new state-of-the-art accuracies on two out of three benchmark datasets, while only ﬁne-tuning a small number of parameters. Further, we show that CSP improves generalization to higher-order attribute-attribute-object compositions and combinations of pretrained attributes and ﬁne-tuned objects. The code is available at https://github.com/BatsResearch/csp.},
	language = {en},
	urldate = {2022-06-06},
	publisher = {arXiv},
	author = {Nayak, Nihal V. and Yu, Peilin and Bach, Stephen H.},
	month = apr,
	year = {2022},
	note = {Number: arXiv:2204.03574
arXiv:2204.03574 [cs]},
	keywords = {Computer Science - Machine Learning, Computer Science - Computation and Language, Computer Science - Computer Vision and Pattern Recognition},
	file = {Nayak et al. - 2022 - Learning to Compose Soft Prompts for Compositional.pdf:/Users/mttrager/Zotero/storage/HKCVAH5C/Nayak et al. - 2022 - Learning to Compose Soft Prompts for Compositional.pdf:application/pdf},
}


@article{caltech256_dataset,
  title={Caltech-256 object category dataset},
  author={Griffin, Gregory and Holub, Alex and Perona, Pietro},
  year={2007},
  publisher={California Institute of Technology}
}

@inproceedings{wang2022learning,
  title={Learning to prompt for continual learning},
  author={Wang, Zifeng and Zhang, Zizhao and Lee, Chen-Yu and Zhang, Han and Sun, Ruoxi and Ren, Xiaoqi and Su, Guolong and Perot, Vincent and Dy, Jennifer and Pfister, Tomas},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={139--149},
  year={2022}
}
